Visual detection of time-varying signals: opposing biases and their timescales

Human visual perception is a complex, dynamic and fluctuating process. In addition to the incoming visual stimulus, it is affected by many other factors including temporal context, both external and internal to the observer. In this study we investigate the dynamic properties of psychophysical responses to a continuous stream of visual near-threshold detection tasks. We manipulate the incoming signals to have temporal structures with various characteristic timescales. Responses of human observers to these signals are analyzed using tools that highlight their dynamical features as well. We find that two opposing biases shape perception, and operate over distinct timescales. Positive recency appears over short times, e.g. consecutive trials. Adaptation, entailing an increased probability of changed response, reflects trends over longer times. Analysis of psychometric curves conditioned on various temporal events reveals that the balance between the two biases can shift depending on their interplay with the temporal properties of the input signal. A simple mathematical model reproduces the experimental data in all stimulus regimes. Taken together, our results support the view that visual response fluctuations reflect complex internal dynamics, possibly related to higher cognitive processes.

==> SignificanceStatement.tex <==
\section*{Author summary}
%}Significance Statement}
%120 words max
\paragraph{}
Human perception exhibits internal dynamics and fluctuates even when external conditions are well controlled. In this study we take the dynamic approach to study these fluctuations, manipulating temporal properties of incoming stream of signals and analyzing dynamic aspects of the responses. Such an approach can reveal internal biases in perception and their characteristic timescales.

We find that human observers exhibit two opposing biases: in the short term they tend to repeat their response, while in the long term they tend to change it. The balance between the two depends on the incoming signal stream. This behavior can be interpreted as an exploration-exploitation trade-off; it suggests that dynamics of perception reflects higher cognitive processes in addition signal detection itself. 
